AdaDeep: A Usage-Driven, Automated Deep Model Compression Framework for Enabling Ubiquitous Intelligent Mobiles

Recent breakthroughs in Deep Neural Networks (DNNs) have fueled a tremendously growing demand for bringing DNN-powered intelligence into mobile platforms. While the potential of deploying DNNs on resource-constrained platforms has been demonstrated by DNN compression techniques, the current practice suffers from two limitations: 1) merely stand-alone compression schemes are investigated even though each compression technique only suit for certain types of DNN layers; and 2) mostly compression techniques are optimized for DNNs' inference accuracy, without explicitly considering other application-driven system performance (e.g., latency and energy cost) and the varying resource availability across platforms (e.g., storage and processing capability). To this end, we propose AdaDeep, a usage-driven, automated DNN compression framework for systematically exploring the desired trade-off between performance and resource constraints, from a holistic system level. Specifically, in a layer-wise manner, AdaDeep automatically selects the most suitable combination of compression techniques and the corresponding compression hyperparameters for a given DNN. Thorough evaluations on six datasets and across twelve devices demonstrate that AdaDeep can achieve up to $18.6\times$ latency reduction, $9.8\times$ energy-efficiency improvement, and $37.3\times$ storage reduction in DNNs while incurring negligible accuracy loss. Furthermore, AdaDeep also uncovers multiple novel combinations of compression techniques.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> body/compress.tex <==
% \section{Tunable Metrics Quantization}
% \label{sec:compression}
To quantify the cost metrics $S$ and $C$ at certain layers using different compression techniques, this section summarizes $9$ types of state-of-the-art layer compression techniques into three categories: weight compression, convolution decomposition, and special layer architecture, present computational equations for $C$ and $S$ based on their application scopes for FC or CONV layers.

Let the input size and the output size of a FC layer be $A$ and $B$, respectively.
Then the weight size and the computation operation of the FC layer are $A \cdot {B}$.
Similarly, denote the input size and the output size of a CONV layer as $M\cdot H_{in}\cdot W_{in}$ and $N\cdot H_{out}\cdot W_{out}$, respectively, where $M$ and $N$ are the channel number of input and output, $H_{in}$, $W_{in}$ are the shape of input features and $H_{out}$, $W_{out}$ show the shape of output features.
Then the weight size and the computation operation of the CONV layer are $M\cdot N\cdot U\cdot V$ and $H_{out}\cdot W_{out}\cdot M\cdot N\cdot U\cdot V$.
\tabref{tb_comp} shows the quantifiable $S$ and $C$ using different compression techniques.
%As next, we review each compression technique in detail.

\begin{table*}[ht]
  \centering
  \scriptsize
  %\tiny
  \caption{Summaries and quantitative analyses of layer compression techniques for NNs.}
  \label{tb_comp}
  \begin{tabular}{|p{46pt}<{\centering}|p{25pt}<{\centering}|p{20pt}<{\centering}|p{136pt}<{\centering}|p{200pt}<{\centering}|}
  \hline
  Type & Method & Layer & Weight size $S_p$ & MAC amounts $C$ \\ \hline
  \multirowcell{2}{Original \\ layer} & N/A & FC & $A \cdot {B}$ & $A\cdot {B}$ \\ \cline{2-5}
  & N/A    &  CONV  & $M \cdot {N} \cdot {U} \cdot {V}$ & $H_{out} \cdot {W_{out}} \cdot {U} \cdot {V} \cdot {N} \cdot {M}$            \\ \hline
  \multirowcell{4}{Weight \\ compression}            & W1~\cite{xue2013restructuring} & FC  & $(A+B)\cdot {k}$  & $(A+B)\cdot {k}$ \\ \cline{2-5}
                                           &W2~\cite{bib:lane2016:sensys} & FC & $  (A+B)\cdot {k}$ & $ (A+B)\cdot {k}$ \\ \cline{2-5}
                                           & W3~\cite{bib:arXiv2015:han} & FC  & $A*B-n_{weight<e}$ &  $A*B-n_{weight<e}$   \\ \cline{2-5}
                                           & W3~\cite{bib:arXiv2015:han} & CONV & $ M \cdot N \cdot U \cdot V - n_{weight<e} $ & $[M \cdot N \cdot U \cdot V - n_{weight<e} ] \cdot H_{out} \cdot W_{out}$  \\ \hline
  \multirowcell{3}{Convolution \\ decomposition} & C1~\cite{bib:cvpr2015:ICCV} & CONV & $(1-\theta) M \cdot {N} \cdot {U} \cdot {V}$ &  $(1-\theta) H_{out}\cdot {W_{out}} \cdot {U} \cdot {V} \cdot {M} \cdot {N} $\\ \cline{2-5} &
C2~\cite{bib:arXiv2017:Howard} & CONV & $\alpha \cdot {M}\cdot {U}\cdot {V}+\alpha ^2 \cdot {M}\cdot {N}$ & $ U \cdot {V} \cdot {\alpha} \cdot {M} \cdot {H_{in}} \cdot {W_{in}}+ \alpha ^2 \cdot {M} \cdot {N} \cdot {H_{in}} \cdot {W_{in}}$ \\ \cline{2-5}
                                           & C3~\cite{bib:ICLR2017:Park} & CONV  & $(1-\alpha) M \cdot {N} \cdot {U} \cdot {V}$ & $(1-\alpha) H_{out}\cdot {W_{out}} \cdot {U} \cdot {V} \cdot {M} \cdot {N} $ \\ \hline
  \multirowcell{3}{Special \\ layer}             & L1~\cite{bib:iandola2016:arxiv} & CONV & $ M_1+   {N_1}+ M_2 \cdot N_2 +(3\cdot {3}\cdot {M_3}\cdot {N_3}) $  & $ H_{out1} \cdot {W_{out1}} \cdot {N_1} \cdot {M_1} + H_{out2} \cdot {W_{out2}} \cdot {N_2} \cdot {M_2} + 3 \cdot 3 \cdot H_{out3} \cdot {W_{out3}} \cdot {N_3} \cdot {M_3} $   \\ \cline{2-5}
                                           & L2~\cite{bib:lin2013:NIN} & CONV & $ {M_1}\cdot {N-1} + M_2 \cdot {N_2} $ &  $ H_{out1} \cdot {W_{out1}} \cdot {U_1} \cdot {V_1}\cdot {N_1} \cdot {M_1} + H_{out2} \cdot {W_{out2}} \cdot {U_2} \cdot {V_1}\cdot {N_2} \cdot {M_2}$ \\ \cline{2-5}
                                           & L3~\cite{bib:lin2013:NIN} & FC & $V\cdot {U}\cdot {M} \cdot {N}$  & $H_{out}\cdot {W_{out}}\cdot {U}\cdot {V}\cdot {N}\cdot {M}$ \\ \hline
\end{tabular}
\end{table*}


\subsection{Weight Compression}
\label{subsec:weight}
Weight compression removes redundant weights to reduce the size of NNs.
It can be applied to compress both FC and CONV layers in CNNs or DNNs.
There are three popular weight compression techniques.
\begin{itemize}
  \item \textbf{Factorization via SVD (W1).}
  It introduces an intermediate layer $L'$ between two adjacent layers $L$ and $L+1$ to compress their trained weights $W$ by Singular Value Decomposition (SVD)~\cite{xue2013restructuring}, and $k$ is the numbers of neurons in the inserted layer $L'$.
  After compression, both the weight size and the computation are reduced to $(A+B)\cdot k$, we set $k=A/12$.%, where $A$ is the number of neurons in $L$.
  \item \textbf{Factorization via Sparse-coding (W2).}
  It decomposes the original weight matrix into two matrices using sparse dictionary learning, where the dictionary with $k$ basis is learned from the original weights $W$ \cite{bib:lane2016:IPSN}.
  With a $k$-basis dictionary, the weight size and the computation of the original layer are reduced to $(A+B)\cdot k$ and $(A+B)\cdot k$.
  W2 is designed to compress FC layers.
  \item
  \textbf{Trained Weight Pruning (W3).}
  It introduces a two-phase compression pipeline (training connectivity,  training weights) to reduce the storage and energy consumption without affecting accuracy~\cite{bib:arXiv2015:han}.
  W3 is applicable for both FC and CONV layers.
  The compressed weight size and computation for FC layers are $A*B-n_{weight<\epsilon}$ and $*B-n_{weight<\epsilon}$, here $n_{weight<\epsilon}$ is the number of unimportant weights below threshold $\epsilon$.
  For CONV layers, the compressed weight size and computation are $ M \cdot N \cdot U \cdot V - n_{weight<e} $ and $[M \cdot N \cdot U \cdot V - n_{weight<e} ] \cdot H_{out} \cdot W_{out}$, respectively.
  %Note that the quantization and encoding techniques in \cite{bib:arXiv2015:han} are excluded in our work.
\end{itemize}
W1 and W2 do not require resource-intensive retraining.
Both methods factorize the original weights by adding a new layer adopting different factorization methods.
Their compression performance is limited by an estimated parameter $k$ for factorization.
W3 usually achieves higher compression ratio than W1 and W2 but requires retraining.

\subsection{Convolution Decomposition}
\label{subsec:convolution}
Convolution operations involve calculations among multiple \textit{channels}, thus incurring intensive computation and memory.
Convolution decomposition techniques compress CONV layers leveraging different types of sparsity in the convolution operation.
We review three representative convolution decomposition methods for CONV layer compression as follows.

\begin{itemize}
  \item \textbf{Convolution Kernel Sparse Decomposition (C1).}
  It maximizes the sparsity of the kernels in convolution operations~\cite{bib:cvpr2015:ICCV}.
  Specifically, a convolution is replaced by its sparse matrix decomposition via principal component analysis.
  The compressed weight size and computation are $(1-\theta) M \cdot N \cdot U \cdot V $ and $(1-\theta) H_{out} \cdot W_{out} \cdot U \cdot V \cdot M \cdot N $ as in \tabref{tb_comp}, where $\theta \in (0,1)$ is the sparsity coefficient.
  \item \textbf{Depth-wise Separable Convolution (C2).}
  It decomposes the standard convolution into a depth-wise convolution and a $1\times{1}$ point-wise convolution~\cite{bib:arXiv2017:Howard}.
  The performance of C2 is controlled by the width multiplier $\alpha$.
  Given a width multiplier $\alpha$, the compressed weight size and computation are $\alpha \cdot M \cdot U \cdot V + \alpha ^2 \cdot M \cdot N$ and $\alpha \cdot U \cdot V \cdot M \cdot H_{in} \cdot W_{in} + \alpha ^2 \cdot M \cdot N \cdot H_{in} \cdot W_{in} $.
  \item \textbf{Sparse Random (C3).}
  The key idea is to replace the dense connections between a small number of channels with sparse connections between a large number of channels for convolution operations~\cite{bib:ICLR2017:soravit}.
  Given a sparsity coefficient $\alpha$, the compressed weight size and computation are $(1-\alpha) M \cdot N \cdot U \cdot V $ and $(1-\alpha) H_{out} \cdot W_{out} \cdot U \cdot V \cdot M \cdot N $.
\end{itemize}

% C1 can aggressively compress the CONV layers in CNNs, while C2 and C3 are useful for large NNs.

\subsection{Special Layer Architecture}
\label{subsec:special}
Instead of layer compression, researchers have also proposed more compact layer architectures.
\begin{itemize}
  \item \textbf{Fire Layer (L1).}
  Fire layers are proposed to replace the CONV layers~\cite{bib:iandola2016:arxiv}.
  A fire layer has a squeeze layer with one filter $M_1 \times N_1 \times 1 \times 1 $, and an expand layer with two filters $M_2 \times N_2 \times 1 \times 1 $ and $M_3 \times N_3 \times 3 \times 3$.
  These three filters are denoted by $s_{1 \times 1}$, $e_{1 \times 1}$ and $e_{3 \times 3}$, whose output sizes are $N_1 \cdot H_{out1}\cdot W_{out1}$, $N_2 \cdot H_{out2}\cdot W_{out2}$ and $N_3 \cdot H_{out3}\cdot W_{out3}$.
  Thus the compressed weight size and computation are $M_1\cdot N_1 + M_2\cdot N_2 + (3 \cdot 3 \cdot M_3 \cdot N_3)$ and $H_{out1} \cdot W_{out1} \cdot M_1 \cdot N_1 + H_{out2} \cdot W_{out2} \cdot M_2 \cdot N_2 + 3\cdot 3 \cdot H_{out3} \cdot W_{out3} \cdot M_3 \cdot N_3$, respectively.
  \item \textbf{MlpConv Layer (L2).}
  It is proposed to increase the depth of CNNs with fewer parameters leveraging a micro multi-layer perceptron embedded with multiple small kernel CONV layers~\cite{bib:lin2013:NIN}.
  Assume there are two layers ($i=1,\,2$) with a norm filter size $M_i \cdot N_i \cdot U_i \cdot V_i$ and output size $H_{outi} \cdot W_{outi} \cdot N_i \cdot M_i$ in the micro network.
  Then the compressed weight size and computation are $ M_1 \cdot N -1 +  M_2 \cdot N_2$ and $\sum_{i=1}^{2}{H_{outi} \cdot W_{outi} \cdot U_i \cdot V_i \cdot M_i \cdot N_i } $.
  \item \textbf{Global Average Pooling Layer (L3).}
  It is introduced to replace the FC layers in CNN to avoid over-fitting~\cite{bib:lin2013:NIN}.
  L3 can replace the FC layer over the feature map to extract the average of each feature map.
  The compressed weight size and computation are $ U \cdot V \cdot M \cdot N \cdot N$ and $H_{out}\cdot W_{out} \cdot U \cdot V \cdot N \cdot M$.
\end{itemize}

% L1 and L2 are suitable to improve the generalization of large CNNs.
% L3 can avoid over-fitting of FC layers and is fit for smaller NNs.
% Combinations of these special layers can further improve the compression performance~\cite{bib:iandola2016:arxiv}\cite{bib:lin2013:NIN}.

The parameters (\ie $k$ in W1 and W2, the depth multiplier $\alpha$ in C2, the sparse random multiplier $\theta$ in C3) are empirically optimized by comparing the performance improvement on the layer where the compression method is applied.
